FORAY: Towards Effective Attack Synthesis against Deep Logical Vulnerabilities in DeFi Protocols

Blockchain adoption has surged with the rise of Decentralized Finance (DeFi) applications. However, the significant value of digital assets managed by DeFi protocols makes them prime targets for attacks. Current smart contract vulnerability detection tools struggle with DeFi protocols due to deep logical bugs arising from complex financial interactions between multiple smart contracts. These tools primarily analyze individual contracts and resort to brute-force methods for DeFi protocols crossing numerous smart contracts, leading to inefficiency. We introduce Foray, a highly effective attack synthesis framework against deep logical bugs in DeFi protocols. Foray proposes a novel attack sketch generation and completion framework. Specifically, instead of treating DeFis as regular programs, we design a domain-specific language (DSL) to lift the low-level smart contracts into their high-level financial operations. Based on our DSL, we first compile a given DeFi protocol into a token flow graph, our graphical representation of DeFi protocols. Then, we design an efficient sketch generation method to synthesize attack sketches for a certain attack goal (e.g., price manipulation, arbitrage, etc.). This algorithm strategically identifies candidate sketches by finding reachable paths in TFG, which is much more efficient than random enumeration. For each candidate sketch written in our DSL, Foray designs a domain-specific symbolic compilation to compile it into SMT constraints. Our compilation simplifies the constraints by removing redundant smart contract semantics. It maintains the usability of symbolic compilation, yet scales to problems orders of magnitude larger. Finally, the candidates are completed via existing solvers and are transformed into concrete attacks via direct syntax transformation.

==> sections/draft0-tech.tex <==
\section{Draft0}

\begin{itemize}
    \item $f = s_0; ...; s_n = \vec{s}$
    \item $f \mapsto e_0; ...; e_m = \vec{e}$
    \item $e = (u,v)$
    \item $e.{\sf src} = u$
    \item $e.{\sf tgt} = v$
    \item $e.{\sf op} = {\sf swap}$
    \item $u.{\sf balance} = \{ v \mapsto x \}$
    \item ${\sf path} = \overrightarrow{\langle e, {\sf params} \rangle}$, two sets of semantics for sketch (abstract) and constraint (domain-specific) generation
    \item ${\sf precedTo}(s_i, s_j)$ can be simplified as $...; s_i; ...; s_j; ...$
    \item TFG construction: flow IR first, then edge and node; no flow will be generated if a statement doesn't match any.
    \item Only tokens are on the graph (static program); parameters and caller (from) receiver (to) are bound to operator (dynamic data) --- they should not be on the graph
    \item $\epsilon$ is a special ACCOUNT, not token.
    \item ``sketch'' is written in AFL, which \textsc{CnstGen} applies; ``program'' is in smart contract language (e.g., Solidity), which can be directly executed.
\end{itemize}

\begin{figure}
    \centering
    \footnotesize
    \begin{mathpar}
    
        \inferrule{
            f \equiv s_0; s_1; ...
        }{
            s_0 \\ s_1 \\ ...
        }\textsc{ (block)}

        \inferrule{
            s \equiv  {\sf if} * {\sf then}\ f_0\ {\sf else}\ f_1
        }{
            f_0 \\ f_1
        }\textsc{ (branch)}

        \inferrule{
            s \equiv u.{\sf transfer}(b, x) \\ a = {\sf this}
        }{
            s : {\sf flow}(u, a, b)
        }\textsc{ (flow-transfer1)}

        \inferrule{
            s \equiv u.{\sf transferFrom}(a, b, x)
        }{
            s : {\sf flow}(u, a, b)
        }\textsc{ (flow-transfer2)}

        \inferrule{
            s \equiv u.{\sf mint}(x) \\\\ a = {\sf this}
        }{
            s : {\sf flow}(u, \epsilon, a)
        }\textsc{ (flow-mint)}

        \inferrule{
            s \equiv b.{\sf burn}(x) \\\\ a = {\sf this}
        }{
            s : {\sf flow}(u, a, \epsilon)
        }\textsc{ (flow-burn)}
        
    \end{mathpar}
    \caption{Flow inference rules. \yanju{$\epsilon$ is a special black hole account (NOT TOKEN) that has infinite number of all tokens, used for expressing special transfer like {\sf mint} and {\sf burn}. For all rules, $a \neq b$ and $a \neq \epsilon$.}}
    \label{draft-fig:inf-flow}
\end{figure}

\begin{figure}
    \centering
    \footnotesize
    \begin{mathpar}

        \inferrule{
            s : {\sf flow}(u, a, b)
        }{
            s : {\sf edge}(u, u, {\sf transfer})
        }\textsc{ (edge-transfer)}

        \inferrule{
            s : {\sf flow}(u, \epsilon, a)
        }{
            s : {\sf edge}(u, u, {\sf mint})
        }\textsc{ (edge-mint)}

        \inferrule{
            s : {\sf flow}(u, a, \epsilon)
        }{
            s : {\sf edge}(u, u, {\sf burn})
        }\textsc{ (edge-burn)}
        
        \inferrule{
            f \equiv ...; s_1; ...; s_2; ... \\ s_1 : {\sf flow}(u, a, b) \\ s_2 : {\sf flow}(v, b, a)
        }{
            s_1 : {\sf edge}(u, v, {\sf swap})
        }\textsc{ (edge-swap)}
        
        \inferrule{
            f \equiv ...; s_1; ...; s_2; ... \\ s_3 \in g \\ {\sf callback}(s_2, g) \\ s_1 : {\sf flow}(u, a, b) \\ s_3: {\sf flow}(u, b, a)
        }{
            {\sf loan}(s_1, s_2, s_3)
        }\textsc{ (pred-loan)}
        
        \inferrule{
            {\sf loan}(s, *, *) \\ s: {\sf flow}(u, a, b)
        }{
            s : {\sf edge}(u, u, {\sf borrow})
        }\textsc{ (edge-borrow)}

        \inferrule{
            {\sf loan}(*, *, s) \\ s: {\sf flow}(u, b, a)
        }{
            s : {\sf edge}(u, u, {\sf payback})
        }\textsc{ (edge-payback)}
        
    \end{mathpar}
    \caption{Edge inference rules.}
    \label{draft-fig:inf-edge}
\end{figure}

\begin{figure}[t!]
    \centering
    \footnotesize
    \begin{mathpar}
        \inferrule{
            {\sf edge}(u, u, {\sf transfer}) \\ a, b, x \in \Phi
        }{
            {\searrow}(t, u, a, x) \cup {\nearrow}(t, u, b, x)
        }\textsc{ (Transfer)}

        \inferrule{
            {\sf edge}(u, u, {\sf burn}) \\ a, x \in \Phi
        }{
            {\searrow}(t, u, a, x)
        }\textsc{ (Burn)}

        \inferrule{
            {\sf edge}(u, u, {\sf mint}) \\ a, x \in \Phi
        }{
            {\nearrow}(t, u, a, x)
        }\textsc{ (Mint)}

        \inferrule{
            {\sf edge}(u, v, {\sf swap}) \\ a, b, x, y \in \Phi
        }{
            {\searrow}(t, u, a, x) \cup {\nearrow}(t, u, b, x) \cup {\searrow}(t, v, b, y) \cup {\nearrow}(t, v, a, y)
        }\textsc{ (Swap)}

        \inferrule{
            {\sf edge}(u, u, {\sf borrow}) \\ a, b, x \in \Phi
        }{
            {\searrow}(t, u, a, x) \cup {\nearrow}(t, u, b, x)
        }\textsc{ (Borrow)}

        \inferrule{
            {\sf edge}(u, u, {\sf payback}) \\ a, b, y \in \Phi
        }{
            {\searrow}(t, u, a, y) \cup {\nearrow}(t, u, b, y) \cup \{ y > x \}
        }\textsc{ (Payback)}\\
        
    \end{mathpar}
    \vspace{-8mm}
    \caption{Domain-specific constraint compilation rules.\yanju{WIP: merge {\sf borrow} and {\sf payback} --- need edge map; need swap equation, swap fees, and other tiny adjustments.}}
    \label{draft-fig:inf-cnst}
\end{figure}

\begin{algorithm}[t]
    \caption{Token Flow Graph Generation}
    \begin{algorithmic}[1]
        \small
        \Procedure{GraphGen}{$D, \phi$} 
            \State {\bf Input:} DeFi $D$, Configuration $\phi$
            \State {\bf Output:} Token Flow Graph $G(N,E)$, Edge Map $Z$
            \State $N, F \gets {\sf tokens}(D), {\sf functions}(D)$
            \State $H \gets \bigcup_{f \in F} \textsc{InferFlows}(\phi, f)$ \Comment{flow analysis}
            \State $Z \gets \textsc{InferEdges}(F, H)$ \Comment{edge analysis}
            \State $E \gets \{ e \mid s : e \in Z \}$ \Comment{edge collection}
            \State \Return $G(N,E)$, $Z$
        \EndProcedure
    \end{algorithmic}
    \label{draft-alg:graphgen}
\end{algorithm}

% \begin{algorithm}[t]
%     \caption{AFL Attack Sketch Enumeration \yanju{Change to constraint-based BFS}}
%     \begin{algorithmic}[1]
%         \small
%         \Procedure{SketchGen}{$G, \phi, \psi$} 
%             \State {\bf Input:} Token Flow Graph $G(N,E)$, Configuration $\phi$, Attack Goal $\psi$
%             \State {\bf Output:} Attack Sketch $R'$ or $\bot$
%             \State $R_0 \gets []$, $S_0 \gets {\sf init}(\phi)$ \Comment{initialize path and state}
%             \State $W \gets [\langle R_0, S_0 \rangle]$ \Comment{initialize worklist}
%             \While {$\langle R, S \rangle \gets W.{\sf deque}()$}
%                 \While {$e, \rho \gets {\sf choose}(E), {\sf choose}(\phi)$}
%                     \State $R' \gets R.{\sf extend}(e)$ \Comment{extend path}
%                     \State $S' \gets \llbracket R' \rrbracket (S, \rho)$ \Comment{evaluate on abstract semantics}
%                     \If {$S' \models \psi$}
%                         \State {\bf yield} $R'$
%                     \EndIf
%                     \State $W.{\sf enque}(\langle R', S' \rangle)$
%                 \EndWhile
%             \EndWhile
%             \State \Return $\bot$
%         \EndProcedure
%     \end{algorithmic}
%     \label{draft-alg:sketchgen}
% \end{algorithm}

\begin{algorithm}[t]
    \caption{AFL Attack Sketch Enumeration \yanju{Change to constraint-based BFS}}
    \begin{algorithmic}[1]
        \small
        \Procedure{SketchGen}{$G, \phi, \psi$} 
            \State {\bf Input:} Token Flow Graph $G(N,E)$, State $S_0$, Attack Goal $\psi$
            \State {\bf Output:} Attack Sketch $R'$ or $\bot$
            \State $R_0 \gets []$ \Comment{initialize path and state}
            \State $W \gets [\langle R_0, S_0 \rangle]$ \Comment{initialize worklist}
            \While {$\langle R, S \rangle \gets W.{\sf deque}()$}
                \While {$e, \rho \gets {\sf choose}(E), {\sf choose}(\phi)$}
                    \State $R' \gets R.{\sf extend}(e)$ \Comment{extend path}
                    \State $S' \gets \llbracket R' \rrbracket (S, \rho)$ \Comment{evaluate on abstract semantics}
                    \If {$S' \models \psi$}
                        \State {\bf yield} $R'$
                    \EndIf
                    \State $W.{\sf enque}(\langle R', S' \rangle)$
                \EndWhile
            \EndWhile
            \State \Return $\bot$
        \EndProcedure
    \end{algorithmic}
    \label{draft-alg:sketchgen}
\end{algorithm}

\begin{algorithm}[t]
    \caption{Attack Synthesis}
    \begin{algorithmic}[1]
    \small 
        \Procedure{\textsc{AtkSyn}}{$D, \phi, \psi$}
            \State \textbf{Input:} DeFi $D$, Configuration $\phi$, Attack goal $\psi$
            \State \textbf{Output:} Attack Program $P$ or $\bot$
            \State $S_0 \gets {\sf init}(\phi)$, $\kappa \gets \varnothing$ \Comment{get initial state and KB}
            \State $G, Z \gets \textsc{GraphGen}(D, \phi)$ \Comment{get token flow graph and edge map}
            \While{$R \gets \textsc{SketchGen}(G, \phi, \psi)$} \Comment{enumerate AFL sketch}
                \State $\delta \gets \bigwedge \textsc{CnstGen}(\phi, R)$ \Comment{generate constraints from sketch}
                \While {$\mu \gets {\sf solve}(\phi \land \psi \land \delta \land \kappa))$} \Comment{get model}
                    \If {$P \gets {\sf complete}(D, \phi, \mu, R, Z)$} \Comment{attack instantiation}
                        \If {$P(S_0) \models \psi$} \Comment{validate attack program $P$}
                            \State \Return $P$
                        \Else
                            \State $\kappa \gets \kappa \land (\bigwedge {\sf muc}(P(S_0) \models \psi))$ \Comment{update KB}
                        \EndIf
                    \EndIf
                \EndWhile
            \EndWhile
            \State \Return $\bot$ \Comment {return when exhausted}
        \EndProcedure
    \end{algorithmic}
    \label{draft-alg:atksyn}
\end{algorithm}

==> sections/draft1-tech.tex <==
\section{Draft1 (Deprecated)}

\begin{figure}
    \centering
    \footnotesize
    \begin{mathpar}
        \inferrule{
             f \equiv s_0; ...; s_n  \\ s_0 : e_0 \\ ... \\ s_n : e_n
        }{
            f:\tfg \rightsquigarrow \tfg \cup e_0 \cup ... \cup e_n
        }\textsc{ (Fun)}

        \inferrule{
             s \equiv {\sf if}\ *\ {\sf then}\ s_0\ {\sf else}\ s_1 \\ s_0: e_0 \\ s_1 : e_1
        }{
            s : \tfg \rightsquigarrow \tfg \cup e_0 \cup e_1
        }\textsc{ (if-else)}
        
        \inferrule{
            s \equiv u.\mathsf{transfer(b,x)} \\ e:\mathsf{edge}(u,\void,\mathsf{transfer},\constraint) \\\\ \constraint \equiv e.i \ge x \land e.o \ge x
        }{
             s : \tfg \rightsquigarrow \tfg \cup e
        }\textsc{ (FlowOut)}
        
        \inferrule{
            s \equiv u.\mathsf{transferFrom}(a,b,x) \\ e:\mathsf{edge}(\void,u,\mathsf{transfer},\constraint) \\\\ \constraint \equiv e.i \ge x \land e.o \ge x 
        }{
             s : \tfg \rightsquigarrow \tfg \cup e
        }\textsc{ (FlowIn)}

        \inferrule{
            s \equiv u.\mathsf{mint}(x) \\ e:\mathsf{edge}(\void,u,\mathsf{mint},\constraint) \\\\ \constraint \equiv e.i < e.o
        }{
            s : \tfg \rightsquigarrow \tfg \cup e
        }\textsc{ (Mint)}

        \inferrule{
        s \equiv u.\mathsf{burn}(x) \\ e:\mathsf{edge}(u,\void,\mathsf{burn},\constraint) \\\\ \constraint \equiv e.i > e.o
        }{
            u.\mathsf{burn}(x) : \tfg \rightsquigarrow \tfg \cup e
        }\textsc{ (Burn)}
        
        \inferrule{
            \constraint \equiv e.i  \odot e.o \\\\  e_1:\mathsf{edge}(u,\void,\mathsf{transfer},\_) \\ e_2:\mathsf{edge}(\void,v,\mathsf{transfer},\_)
        }{
            e:\mathsf{edge}(u,v,\mathsf{swap},\constraint), \tfg \rightsquigarrow \tfg \cup e \setminus e_1 \setminus e_2
        }\textsc{ (Swap)}
        
        {\scriptsize 
        \inferrule{
            s_1:e_1:\mathsf{edge}(\void,u,\mathsf{transfer},\_) \\ \mathsf{callback}(s_2, g) \\  s3:e_2:\mathsf{edge}(u,\void,\mathsf{transfer},\_)  \\ f, g \in \fundom \\ s_1, s_2 \in f \\ s_3 \in g \\ \mathsf{precedeTo}(s_1, s_2) \\ \mathsf{precedeTo}(s_2, s_3)
        }{
            \mathsf{loan}(s_1,s_2,s_3)
        }\textsc{ (Loan)}
        }
        
        \inferrule{
            \mathsf{loan}(s,\_,\_) \\ \constraint \equiv e'.i > 0 \land e'.o > 0 \\\\ e: \mathsf{edge}(\void, u,\mathsf{transfer},\_)
        }{
           e': \mathsf{edge}(\void, u,\mathsf{borrow},\constraint), \tfg \rightsquigarrow \tfg \cup e' \setminus e
        }\textsc{ (Borrow)}

        \inferrule{
            \mathsf{loan}(\_,\_,s) \\ \constraint \equiv e'.i > 0 \land e'.o > 0 \\\\ e: \mathsf{edge}(u,\void,\mathsf{transfer},\_)
        }{
             e': \mathsf{edge}(u,\void, \mathsf{payback},\constraint),\tfg \rightsquigarrow \tfg \cup e' \setminus e
        }\textsc{ (Payback)}
        
    \end{mathpar}
    \caption{Inference rules for constructing TFG. $e.i$ and $e.o$ denote the input and output node of an edge $e$.
    The predicates are defined in Table~\ref{tab:preds}.
    Each rule can be interpreted as: if the conditions above the line satisfied, the function (left part below the line) is equivalent to a certain set of graph operations (right part below the line), which adds or deletes certain edges from $\tfg$.
    }
    \vspace{-5mm}
    \label{draft1-fig:inf-tfg}
\end{figure}

==> sections/draft2-tech.tex <==
\section{Draft2}

% \begin{figure}
%     \centering
%     \footnotesize
%     \begin{mathpar}
    
%         \inferrule{
%             f \equiv s_0; s_1; ...
%         }{
%             s_0 \\ s_1 \\ ...
%         }\textsc{ (seq)}

%         \inferrule{
%             s \equiv  {\sf if}\ \_\ {\sf then}\ f_0\ {\sf else}\ f_1
%         }{
%             f_0 \\ f_1
%         }\textsc{ (branch)}

%         \inferrule{
%             s \equiv u.{\sf transfer}(b, x) \\\\ a = {\sf this}
%         }{
%             s : {\sf flow}(u, x, a, b)
%         }\textsc{ (flow-out)}

%         \inferrule{
%             s \equiv u.{\sf transferFrom}(a, b, x)
%         }{
%             s : {\sf flow}(u, x, a, b)
%         }\textsc{ (flow-in)}

%         \inferrule{
%             s \equiv u.{\sf mint}(x) \\\\ a = {\sf this}
%         }{
%             s : {\sf flow}(u, x, \bullet, a)
%         }\textsc{ (flow-mint)}

%         \inferrule{
%             s \equiv b.{\sf burn}(x) \\\\ a = {\sf this}
%         }{
%             s : {\sf flow}(u, x, a, \bullet)
%         }\textsc{ (flow-burn)}
        
%     \end{mathpar}
%     \caption{Flow inference rules.}
%     \label{draft-fig:inf-flow}
% \end{figure}

\begin{figure}
    \centering
    \footnotesize
    \begin{mathpar}

        \inferrule{
            f \equiv s_0; ...; s_n \\\\ \langle \mathbb{W}_f, s_0 \rangle \rightsquigarrow \langle \mathbb{W}_0, {\sf void} \rangle \\ ... \\ \langle \mathbb{W}_{n-1}, s_n \rangle \rightsquigarrow \langle \mathbb{W}_n, {\sf void} \rangle
        }{
            \langle \mathbb{W}_0, f \rangle \rightsquigarrow \langle \mathbb{W}_n , {\sf void} \rangle
        }\textsc{ (fun)}

        \inferrule{
             s \equiv  {\sf if}\ \_\ {\sf then}\ f_0\ {\sf else}\ f_1 \\\\ \langle \mathbb{W}_s, f_0 \rangle \rightsquigarrow \langle \mathbb{W}_0, {\sf void} \rangle \\ \langle \mathbb{W}_s, f_1 \rangle \rightsquigarrow \langle \mathbb{W}_1, {\sf void} \rangle
        }{
            \langle \mathbb{W}_s, s \rangle \rightsquigarrow \langle \mathbb{W}_0 \cup \mathbb{W}_1, {\sf void} \rangle
        }\textsc{ (branch)}

        \inferrule{
            s \equiv u.{\sf transfer}(b, x) \\ a = {\sf this} \\ w \equiv {\sf flow}(u, x, a, b)
        }{
            \langle \mathbb{W}_s, s \rangle \rightsquigarrow \langle \mathbb{W}_s \cup \{s:w\}, {\sf void} \rangle
        }\textsc{ (flow-out)}

        \inferrule{
            s \equiv u.{\sf transferFrom}(a, b, x) \\ w \equiv {\sf flow}(u, x, a, b)
        }{
            \langle \mathbb{W}_s, s \rangle \rightsquigarrow \langle \mathbb{W}_s \cup \{s:w\}, {\sf void} \rangle
        }\textsc{ (flow-in)}

        \inferrule{
            s \equiv u.{\sf mint}(x) \\ a = {\sf this} \\ w \equiv {\sf flow}(u, x, \bullet, a)
        }{
            \langle \mathbb{W}_s, s \rangle \rightsquigarrow \langle \mathbb{W}_s \cup \{s:w\}, {\sf void} \rangle
        }\textsc{ (flow-mint)}

        \inferrule{
            s \equiv b.{\sf burn}(x) \\ a = {\sf this} \\ w \equiv {\sf flow}(u, x, a, \bullet)
        }{
            \langle \mathbb{W}_s, s \rangle \rightsquigarrow \langle \mathbb{W}_s \cup \{s:w\} \rangle
        }\textsc{ (flow-burn)}

    \end{mathpar}
    \caption{Flow inference rules.}
    \label{draft-fig:inf-flow}
\end{figure}

\begin{figure}
    \centering
    \footnotesize
    \begin{mathpar}

        \inferrule{
            s : {\sf flow}(u, x, a, b) \in \mathbb{W} \\ \Phi \equiv u[a] \geq x \land u'[a] \leq u[a]
        }{
            {\sf edge}(u, \epsilon, {\sf transfer}, \Phi)
        }\textsc{ (edge-transfer)}

        \inferrule{
            s : {\sf flow}(u, x, \bullet, a) \in \mathbb{W} \\ \Phi \equiv u'[a] \geq x \land u'[a] \geq u[a]
        }{
            {\sf edge}(\epsilon, u, {\sf mint}, \Phi)
        }\textsc{ (edge-mint)}

        \inferrule{
            s : {\sf flow}(u, x, a, \bullet) \in \mathbb{W} \\ \Phi \equiv u[a] \geq x \land u'[a] \leq u[a]
        }{
            {\sf edge}(u, \epsilon, {\sf burn}, \Phi)
        }\textsc{ (edge-burn)}
        
        \inferrule{
            f \equiv ...; s_1; ...; s_2; ... \\\\ s_1 : {\sf flow}(u, x, a, b) \in \mathbb{W} \\ s_2 : {\sf flow}(v, y, b, a) \in \mathbb{W} \\\\ \Phi \equiv u[a] \geq x \land u'[a] \leq u[a] \land v'[a] \geq y \land v'[a] \geq v[a]
        }{
            {\sf edge}(u, v, {\sf swap}, \Phi)
        }\textsc{ (edge-swap)}
        
        \inferrule{
            f \equiv ...; s_1; ...; s_2; ... \\ s_3 \in g \\ {\sf callback}(s_2, g) \\\\ s_1 : {\sf flow}(u, x, a, b) \in \mathbb{W} \\ s_3: {\sf flow}(u, y, b, a) \in \mathbb{W}
        }{
            {\sf loan}(s_1, s_2, s_3)
        }\textsc{ (loan)}
        
        \inferrule{
            {\sf loan}(s, \_, \_) \\ s: {\sf flow}(u, x, b, a) \in \mathbb{W} \\\\ \Phi \equiv u'[a] \geq x \land u'[a] \geq u[a]
        }{
            {\sf edge}(\epsilon, u, {\sf borrow}, \Phi)
        }\textsc{ (edge-borrow)}

        \inferrule{
            {\sf loan}(\_, \_, s) \\ s: {\sf flow}(u, x, a, b) \in \mathbb{W} \\\\ \Phi \equiv u[a] \geq x \land u'[a] \leq u[a]
        }{
            {\sf edge}(u, \epsilon, {\sf payback}, \Phi)
        }\textsc{ (edge-payback)}
        
    \end{mathpar}
    \caption{Edge inference rules.$u[a]$ is the user $a$'s balance of token $u$ at current time step; $u'[a]$ is the updated balance after executing $e.{\sf op}$. Perspective is fixed to $a$. $\epsilon$ is a token, and $\bullet$ is a special/blackhole account of $\epsilon$ token.}
    \label{draft-fig:inf-edge}
\end{figure}

% \begin{algorithm}[t]
%     \caption{Attack Sketch Enumeration}
%     \begin{algorithmic}[1]
%         \small
%         \Procedure{SketchGen}{$S_0, \psi, \tfg$} 
%             \State {\bf Input:} Initial State $S_0$, Attack Goal $\psi$, Token Flow Graph $\tfg$
%             \State {\bf Output:} Attack Sketch $\tilde{P}$ or $\bot$
            
%             \State {\bf Assume} $\tfg = (\token,\afl, \edgedom, M_0, \constraint)$
%             \State $R_0, \cststore_0 \gets [], {\sf init}(\tfg, S_0)$ \Comment{init. reachable path \& constraint store}
%             \State $W \gets \{ \langle R_0, \cststore_0 \rangle \}$ \Comment{initialize priority worklist}
            
%             \While{$\langle R, \cststore \rangle \gets W.{\sf pop}()$} \Comment{choose a path-constraint pair}
%                 \State $N \gets \{ \epsilon \} \cup (\bigcup_{e \in R} \{ u, v \mid e \equiv (u, v, *, *) \})$ \Comment{nodes covered}
%                 \State $E \gets \bigcup_{n \in N, e \in R} \{ e \mid e \equiv (n, *, *, *) \}$ \Comment{neighboring edges}
%                 \ForAll{$e \in E$}
%                     \State $\cststore' \gets \cststore \land e.\constraint$ \Comment{update constraints}
%                     \State {\bf if} ${\sf unsat}(\cststore')$ {\bf then} {\bf continue}
%                     \State $N' \gets ??$ \Comment{update covered nodes}
%                     \If {$\rho(\psi) \subseteq N'$} \Comment{projection of attack goal to markings?}
%                         \State $R' \gets R + [e]$ \Comment{add edge to path}
%                         \State $\tilde{P} \gets ( e.{\sf op} \mid \forall e \in R')$ \Comment{get sketch}
%                         \State {\bf yield} $\tilde{P}$
%                     \EndIf
%                     \State $W.{\sf push}(\langle R', \cststore' \rangle)$ \Comment{update priority worklist}
            
%                 \EndFor
%             \EndWhile
%             \State \Return $\bot$
%         \EndProcedure
%     \end{algorithmic}
%     \label{draft-alg:sketch-generation}
% \end{algorithm}

\begin{algorithm}[t]
    \caption{Attack Sketch Enumeration}
    \begin{algorithmic}[1]
        \small
        \Procedure{SketchGen}{$S_0, \psi, \tfg, \kappa$} 
            \State {\bf Input:} Initial State $S_0$, Attack Goal $\psi$,
            \Statex \phantom{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ } Token Flow Graph $\tfg$, Knowledge Base $\kappa$
            \State {\bf Output:} Attack Sketch $\tilde{P}$ or $\bot$
            \State {\bf Assume:} $\tfg = (\token, \afl, \edgedom, \constraint)$

            \State $R \gets \{\}$ \Comment{initialize reachable path as ordered set}
            \State $W, \Omega \gets {\sf init}(\tfg, S_0)$ \Comment{initialize worklist $W$ and constraint store $\Omega$}

            \While {${\sf\bf choose}\ t \in W$} \Comment{choose and remove a token from $W$}
                \State $E \gets \{ e \mid \forall e \in \edgedom\ .\ e \equiv {\sf edge}(t, *, *, *) \}$ \Comment{neighboring edges}
                \ForEach {$e \in E$}
                    \State {\bf if} ${\sf unsat}(\Omega \land \kappa \land e.\Phi)$ {\bf then} {\bf continue}
                    \State $W \gets W \cup \{ e.{\sf out} \}$ \Comment{include output node to worklist}
                    \State $\Omega \gets \Omega \land e.\Phi$ \Comment{update constraint store}
                    \State $R \gets R \cup \{ e \}$ \Comment{add edge to reachable path}
                    \If {$\alpha(\psi) \subseteq W$} 
                        \State $\tilde{P} \gets (e.{\sf op} \mid \forall e \in R)$ \Comment{convert graph to sketch}
                        \State \Return $\tilde{P}$
                    \EndIf
                \EndFor
            \EndWhile
            
            \State \Return $\bot$
        \EndProcedure
    \end{algorithmic}
    \label{draft-alg:sketch-generation}
\end{algorithm}

\begin{algorithm}[t]
    \caption{Attack Synthesis}
    \begin{algorithmic}[1]
    \small 
        \Procedure{\textsc{AtkSyn}}{$D, S_0, \psi$}
            \State \textbf{Input:} DeFi $D$, Initial State $S_0$, Attack Goal $\psi$
            \State \textbf{Output:} Attack Program $P$ or $\bot$
            \State $\kappa \gets \varnothing$ \Comment{initialize knowledge base}
            \State $\tfg \gets \textsc{GraphGen}(D, S_0)$ \Comment{construct token flow graph}
            \While{$\tilde{P} \gets \textsc{SketchGen}(S_0, \psi, \tfg, \kappa)$} \Comment{enumerate AFL sketch}
                \State $\delta \gets \textsc{CnstGen}(\phi, R)$ \Comment{generate constraints from sketch}
                \While {$\mu \gets {\sf solve}(S_0 \land \psi \land \kappa \land \delta))$} \Comment{get model}
                    \If {$P \gets {\sf complete}(S_0, \tilde{P}, \mu)$} \Comment{attack instantiation}
                        \If {$P(S_0) \models \psi$} \Comment{validate attack program $P$}
                            \State \Return $P$
                        \Else
                            \State $\kappa \gets \kappa \land \lnot {\sf muc}(P(S_0) \models \psi)$ \Comment{update KB}
                        \EndIf
                    \EndIf
                \EndWhile
            \EndWhile
            \State \Return $\bot$
        \EndProcedure
    \end{algorithmic}
    \label{draft-alg:attack-synthesis}
\end{algorithm}


\begin{figure}[t!]
    \centering
    \footnotesize
    \begin{mathpar}
        \inferrule{
            \mathsf{transfer}(u,a,b,x)
        }{
            {\downarrow}(t, u, a, x) \land {\uparrow}(t, u, b, x)
        }\textsc{ (transfer)}

        \inferrule{
            \mathsf{burn}(u,a,x)
        }{
            {\downarrow}(t, u, a, x)
        }\textsc{ (burn)}

        \inferrule{
            \mathsf{mint}(u,a,x)
        }{
            {\uparrow}(t, u, a, x)
        }\textsc{ (mint)}

        \inferrule{
            \mathsf{swap}(a,u,v,x,y,b)
        }{
            \varsigma(a, u, v, x, y, b) \land \rho(x, y)
        }\textsc{ (swap)}

        \inferrule{
            \mathsf{borrow}(u,a,b,x)
        }{
            {\downarrow}(t, u, a, x) \land {\uparrow}(t, u, b, x)
        }\textsc{ (borrow)}

        \inferrule{
            \mathsf{payback}(u,a,b,y)
        }{
            {\downarrow}(t, u, a, y) \land {\uparrow}(t, u, b, y) \land \vartheta(x,y)
        }\textsc{ (payback)}
        
    \end{mathpar}
    \caption{Domain-specific constraint compilation rules. $\varsigma$ denotes constraints for {\sf swap}, which is $\varsigma(a, u, v, x, y, b): {\downarrow}(t, u, a, x) \land {\uparrow}(t, u, b, x) \land {\downarrow}(t, v, b, y) \land {\uparrow}(t, v, a, y)$, and $\rho$ denotes price exchange model. A typical $\rho$ can be $\rho(x,y): x * y = k$. Other fees can be expressed by $\vartheta$. A typical $\vartheta$ can be $\vartheta(x,y): y > x$, indicating that applying fees on $x$ gets $y$.}
    \label{draft-fig:inf-constraints}
\end{figure}

\begin{figure}[!t]
    \centering
    \begin{align*}
        \psi ::= \exists x. \psi \mid \lnot \psi \mid \psi \land \psi
    \end{align*}
    \caption{Syntax for attack goal.}
    \label{draft-fig:atk-lang}
\end{figure}
